Discovering Structure From Corruption for Unsupervised Image Reconstruction

We consider solving ill-posed imaging inverse problems without access to an image prior or ground-truth examples. An overarching challenge in these inverse problems is that an infinite number of images, including many that are implausible, are consistent with the observed measurements. Thus, image priors are required to reduce the space of possible solutions to more desirable reconstructions. However, in many applications it is difficult or potentially impossible to obtain example images to construct an image prior. Hence inaccurate priors are often used, which inevitably result in biased solutions. Rather than solving an inverse problem using priors that encode the spatial structure of any one image, we propose to solve a set of inverse problems jointly by incorporating prior constraints on the collective structure of the underlying images. The key assumption of our work is that the underlying images we aim to reconstruct share common, low-dimensional structure. We show that such a set of inverse problems can be solved simultaneously without the use of a spatial image prior by instead inferring a shared image generator with a low-dimensional latent space. The parameters of the generator and latent embeddings are found by maximizing a proxy for the Evidence Lower Bound (ELBO). Once identified, the generator and latent embeddings can be combined to provide reconstructed images for each inverse problem. The framework we propose can handle general forward model corruptions, and we show that measurements derived from only a small number of ground-truth images ($\leqslant 150$) are sufficient for image reconstruction. We demonstrate our approach on a variety of convex and non-convex inverse problems, including denoising, phase retrieval, and black hole video reconstruction.

==> sections/appx_experimental_details.tex <==
\section{Experimental details}
\label{appx:supplementary-exp-details}

 \paragraph{Model selection} We parameterize the latent variational distributions $q_{\phi}(z)$ with normalizing flows $l_{\phi}$. In particular, suppose our latent variables $z = l_{\phi}(s)$ where $s \sim \mathcal{N}(0,I)$. Then, \begin{align*}
     \log q_{\phi}(z) = \log \pi (s) - \log\left|\det\frac{dl_{\phi}(s)}{ds}\right|
 \end{align*} where $\pi(\cdot)$ denotes the likelihood of the base distribution of $s$, which in this case is a Gaussian. For our prior on $z$ given $G_{\theta}$, we use an isotropic Gaussian prior. Then the $\ELBOProxy$ equation becomes \begin{align*}
    \ELBOProxy(G_{\theta}, q_{\phi}; y) & := \E_{z \sim l_{\phi}(z)} [\log p(y|G(z)) \\
    & + \log p(z|G) - \log q_{\phi}(z)] \\
    & = \E_{s \sim \mathcal{N}(0,I)} \Big[\log p(y|G_{\theta}(l_{\phi}(s))) \\
    & + \frac{1}{2}\|l_{\phi}(s)\|^2_2 - \log \pi (s) \\
    & + \log\left|\det\frac{dl_{\phi}(s)}{ds}\right|\Big].
 \end{align*} Since the expectation over $\log\pi(s)$ is constant with respect to the parameters $\phi$, we arrive at  
 \begin{align*}
   \ELBOProxy(G_{\theta}, q_{\phi}; y) & = \E_{s \sim \mathcal{N}(0,I)} \Big[\log p(y|G(l_{\phi}(s))) \\
   & + \frac{1}{2}\|l_{\phi}(s)\|^2_2  \\
 & + \log\left|\det\frac{dl_{\phi}(s)}{ds}\right|\Big].
 \end{align*}

\paragraph{Learning the IGM} 

We parameterize the posterior using Gaussian distributions due to memory constraints; the memory of the whole setup with Normalizing Flows using 75 images is around 5 times larger than the setup using a Gaussian variational family.  Note that we do not notice overfitting so there is no need for early stopping.

We train for 99,000 epochs using the Adam \cite{kingma2014adam} optimizer with a learning rate of 1e-4, which takes around 54 hours for 75 images and 4 hours for 4 images on a single NVIDIA A100 GPU. We use a batch size of 20 samples per measurement $i$, and we perform batch gradient descent based on all measurements $i \in \{1, \dots, N\}$.


==> sections/appx_theory.tex <==
\section{Supplemental theoretical results}
\label{appx:supplementary-theory}


\subsection{Proof of Proposition \ref{prop:ELBOProxy_equivalence}}

Let $p_Z$ denote the base distribution of $G$. We will prove that \begin{align*}
    \mathbb{E}_{x \sim h_{\phi}(x)}[\log p(x|G) & - \log h_{\phi}(x)] \\
    & = \mathbb{E}_{z \sim q_{\phi}(z)}[\log p_Z(z) - \log q_{\phi}(z)]
\end{align*} Let $J_{G}(z) \in \R^{n \times k}$ denote the Jacobian of $G$ at an input $z$.  Since $G$ is injective, we can compute the likelihood of a point in the range of $G$ \cite{kothari2021trumpets} via \begin{align*}
    \log p(x|G) & = \log p_Z(G^{\dagger}(x)) \\
   &  - \frac{1}{2}\log|\det[J_G(G^{\dagger}(x))^TJ_G(G^{\dagger}(x))]|
\end{align*} where $G^{\dagger}$ is the inverse of $G$ on its range. Likewise, since $h_{\phi}$ is the push-forward of $q_{\phi}(z)$ through $G$, we can compute the entropy as \begin{align*}
    \log h_{\phi}(x) & = \log q_{\phi}(G^{\dagger}(x)) \\
   &  - \frac{1}{2}\log|\det[J_G(G^{\dagger}(x))^TJ_G(G^{\dagger}(x))]|.
\end{align*} Thus, for $x \in \mathrm{range}(G)$, we have that \begin{align*}
    \log p(x|G) - \log h_{\phi}(x) = \log p_Z(G^{\dagger}(x)) - \log q_{\phi}(G^{\dagger}(x)).
\end{align*} Observe, then that for $x \sim h_{\phi}(x)$, $x = G(z)$ for some $z \sim q_{\phi}(z)$, giving $G^{\dagger}(x) = G^{\dagger}(G(z)) = z$. Thus, \begin{align*}
    \mathbb{E}_{x \sim h_{\phi}(x)}& [\log p(x|G)  - \log h_{\phi}(x)] \\
    & = \mathbb{E}_{x \sim h_{\phi}(x)}[\log p_Z(G^{\dagger}(x)) - \log q_{\phi}(G^{\dagger}(x))] \\
    & =\mathbb{E}_{z \sim q_{\phi}(z)}[\log p_Z(G^{\dagger}(G(z))) - \log q_{\phi}(G^{\dagger}(G(z)))] \\
    & = \mathbb{E}_{z \sim q_{\phi}(z)}[\log p_Z(z) - \log q_{\phi}(z)].
\end{align*} 

\subsection{Proof of Proposition \ref{prop:loss_closed_form}}

Since the loss is separable in $N$, we can consider computing the loss for a single $i \in [N]$. Dropping the indices for notational simplicity, consider a fixed $y = Ax + \eta \in \R^m$ where $\eta \sim \Ncal(0,\sigma^2I_m)$. We aim to calculate \begin{align*}
     \E_{v}\left[- \log p(y | G_m(v)) - \log p(v |G_m) + \log q_{\phi}(v)\right].
\end{align*} Note that $v \sim q_{\phi} = \Ncal(\mu, UU^T)$ is equivalent to $v = Uz + \mu$ for $z \sim \mathcal{N}(0,I_k)$. We can calculate the individual terms in the loss as follows. We first collection some useful results, whose proof can be found in the Supplemental material:
\begin{lemma} \label{lem:helpful-expectations}
For any matrix $U \in \R^{d \times k}$, we have $\E_z\|Uz\|_2^2 = \|U\|_F^2$ where $z \sim \mathcal{N}(0,I_k)$. Moreover, if $UU^T$ is invertible, then $\E_z[z^TU^T(UU^T)^{-1}Uz] = d$.
\end{lemma}

Now, for the first term, since the noise is Gaussian with variance $\sigma^2$, it is equal to \begin{align*}
     \E_z\frac{1}{2\sigma^2}\|y & - AG_m(Uz + \mu)\|_2^2  = \frac{1}{2\sigma^2}\|y\|_2^2 \\
     &+ \E_z\frac{1}{2\sigma^2}\|AG_m(Uz + \mu)\|_2^2 \\
     & - \frac{1}{\sigma^2}\E_z\langle y, AG_m(Uz + \mu)\rangle \\
    & = \frac{1}{2\sigma^2}\left(\|y\|_2^2 + \|AG_mU\|_F^2 + \|AG_m\mu\|_2^2\right) \\
    & - \frac{1}{\sigma^2} \langle y, AG_m \mu\rangle
\end{align*} where we used the first part of Lemma \ref{lem:helpful-expectations} in the third equality. For the prior term, we can calculate using Lemma \ref{lem:helpful-expectations} again

 \begin{align*}
    \E_{v }\left[- \log p(v | G_m)\right] & = \E_z\frac{1}{2}\|Uz + \mu\|_2^2 \\
    & = \frac{1}{2}(\|U\|_F^2 + \|\mu\|_2^2).
\end{align*} Finally, we can calculate the entropy term as

 \begin{align*}
    \E_{v}& \left[\log q_{\phi}(v)\right] = - \frac{1}{2}\E_{v }\left[(v - \mu)^T(UU^T)^{-1}(v-\mu)\right] \\
    & - \frac{k}{2}\log (2\pi) - \frac{1}{2}\log|\det(UU^T)| \\
    & =  - \frac{1}{2}\E_{z}\left[(Uz +\mu - \mu)^T(UU^T)^{-1}(Uz + \mu-\mu)\right] \\
    & - \frac{k}{2}\log (2\pi) - \frac{1}{2}\log|\det(UU^T)| \\
    & = - \frac{1}{2}\E_{z}\left[z^TU^T(UU^T)^{-1}Uz\right] \\
    & - \frac{k}{2}\log (2\pi) - \frac{1}{2}\log|\det(UU^T)| \\
    & =  -\frac{k}{2}- \frac{k}{2}\log (2\pi) - \log\det(U)
\end{align*} where we used the second half of Lemma \ref{lem:helpful-expectations} in the last equality and $\log |\det(UU^T)| = 2\log \det(U)$ in the last equality. Adding the terms achieves the desired result.
